How Deep is your Learning: the DL-HARD Annotated Deep Learning Dataset

Deep Learning Hard (DL-HARD) is a new annotated dataset designed to more effectively evaluate neural ranking models on complex topics. It builds on TREC Deep Learning (DL) topics by extensively annotating them with question intent categories, answer types, wikified entities, topic categories, and result type metadata from a commercial web search engine. Based on this data, we introduce a framework for identifying challenging queries. DL-HARD contains fifty topics from the official DL 2019/2020 evaluation benchmark, half of which are newly and independently assessed. We perform experiments using the official submitted runs to DL on DL-HARD and find substantial differences in metrics and the ranking of participating systems. Overall, DL-HARD is a new resource that promotes research on neural ranking methods by focusing on challenging and complex topics.

==> tables/2020_runs_dl_vs_dl_hard.tex <==
\begin{table*}[]
\caption{System effectiveness on \HARD\ compared with DL track for the 2020 document ranking task.}
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|}
\cline{2-10}
\label{tab:2020_runs_dl_vs_dl_hard}

                                                 & \multicolumn{3}{c|}{\textbf{NDCG@10}}                                                                                  & \multicolumn{3}{c|}{\textbf{RR}}                                                                                       & \multicolumn{3}{c|}{\textbf{Recall@100}}                                                                               \\ \hline
\multicolumn{1}{|l|}{\textbf{name}}              & \multicolumn{1}{l|}{\textbf{\HARD}} & \multicolumn{1}{l|}{\textbf{DL Track}} & \multicolumn{1}{l|}{\textbf{\% Diff}} & \multicolumn{1}{l|}{\textbf{\HARD}} & \multicolumn{1}{l|}{\textbf{DL Track}} & \multicolumn{1}{l|}{\textbf{\% Diff}} & \multicolumn{1}{l|}{\textbf{\HARD}} & \multicolumn{1}{l|}{\textbf{DL Track}} & \multicolumn{1}{l|}{\textbf{\% Diff}} \\ \hline
\multicolumn{1}{|l|}{\textbf{ICIP\_run1}}        & 0.452                                 & 0.662                                  & -21.1\%                               & 0.510                                 & 0.736                                  & -22.7\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{d\_d2q\_duo}}       & 0.449                                 & 0.693                                  & -24.5\%                               & 0.472                                 & 0.734                                  & -26.2\%                               & 0.690                                 & 0.842                                  & -15.3\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{fr\_doc\_roberta}}  & 0.442                                 & 0.640                                  & -19.9\%                               & 0.524                                 & 0.733                                  & -20.9\%                               & 0.641                                 & 0.788                                  & -14.6\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{d\_d2q\_rm3\_duo}}  & 0.438                                 & 0.690                                  & -25.2\%                               & 0.479                                 & 0.735                                  & -25.6\%                               & 0.664                                 & 0.860                                  & -19.6\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{mpii\_run2}}        & 0.432                                 & 0.613                                  & -18.1\%                               & 0.468                                 & 0.677                                  & -20.9\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{bcai\_bertb\_docv}} & 0.431                                 & 0.628                                  & -19.6\%                               & 0.416                                 & 0.739                                  & -32.3\%                               & 0.581                                 & 0.760                                  & -17.9\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{ICIP\_run3}}        & 0.431                                 & 0.653                                  & -22.2\%                               & 0.536                                 & 0.755                                  & -21.9\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{bigIR-DTH-T5-F}}    & 0.425                                 & 0.591                                  & -16.5\%                               & 0.559                                 & 0.681                                  & -12.1\%                               & 0.581                                 & 0.736                                  & -15.5\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{d\_rm3\_duo}}       & 0.424                                 & 0.679                                  & -25.5\%                               & 0.467                                 & 0.733                                  & -26.6\%                               & 0.622                                 & 0.826                                  & -20.4\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{ndrm3-full}}        & 0.415                                 & 0.616                                  & -20.1\%                               & 0.448                                 & 0.716                                  & -26.8\%                               & 0.609                                 & 0.780                                  & -17.1\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{ICIP\_run2}}        & 0.413                                 & 0.632                                  & -21.9\%                               & 0.489                                 & 0.733                                  & -24.4\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{ndrm3-re}}          & 0.409                                 & 0.616                                  & -20.7\%                               & 0.455                                 & 0.713                                  & -25.9\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{roberta-large}}     & 0.408                                 & 0.629                                  & -22.2\%                               & 0.465                                 & 0.739                                  & -27.4\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{mpii\_run1}}        & 0.407                                 & 0.602                                  & -19.4\%                               & 0.494                                 & 0.696                                  & -20.2\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{bigIR-DTH-T5-R}}    & 0.407                                 & 0.603                                  & -19.6\%                               & 0.507                                 & 0.697                                  & -19.0\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{bigIR-DH-T5-F}}     & 0.404                                 & 0.573                                  & -16.9\%                               & 0.572                                 & 0.659                                  & -8.8\%                                & 0.581                                 & 0.736                                  & -15.5\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{ndrm3-orc-full}}    & 0.402                                 & 0.625                                  & -22.3\%                               & 0.486                                 & 0.719                                  & -23.3\%                               & 0.611                                 & 0.784                                  & -17.3\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{ndrm3-orc-re}}      & 0.397                                 & 0.622                                  & -22.5\%                               & 0.419                                 & 0.692                                  & -27.3\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{TUW-TKL-2k}}        & 0.396                                 & 0.585                                  & -18.9\%                               & 0.462                                 & 0.689                                  & -22.7\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{TUW-TKL-4k}}        & 0.393                                 & 0.575                                  & -18.2\%                               & 0.486                                 & 0.694                                  & -20.8\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{bigIR-DH-T5-R}}     & 0.392                                 & 0.585                                  & -19.3\%                               & 0.521                                 & 0.681                                  & -16.0\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{ndrm1-full}}        & 0.382                                 & 0.599                                  & -21.8\%                               & 0.451                                 & 0.726                                  & -27.5\%                               & 0.479                                 & 0.722                                  & -24.2\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{ndrm1-re}}          & 0.377                                 & 0.616                                  & -23.9\%                               & 0.450                                 & 0.725                                  & -27.6\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{indri-sdmf}}        & 0.376                                 & 0.560                                  & -18.3\%                               & 0.423                                 & 0.652                                  & -22.9\%                               & 0.512                                 & 0.739                                  & -22.7\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{d\_d2q\_bm25}}      & 0.372                                 & 0.589                                  & -21.6\%                               & 0.476                                 & 0.697                                  & -22.1\%                               & 0.623                                 & 0.759                                  & -13.5\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{uob\_runid3}}       & 0.371                                 & 0.595                                  & -22.4\%                               & 0.531                                 & 0.710                                  & -18.0\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{longformer\_1}}     & 0.363                                 & 0.552                                  & -18.9\%                               & 0.439                                 & 0.678                                  & -23.8\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{uob\_runid2}}       & 0.363                                 & 0.583                                  & -22.0\%                               & 0.486                                 & 0.715                                  & -22.9\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{uogTrQCBMP}}        & 0.360                                 & 0.579                                  & -21.9\%                               & 0.480                                 & 0.719                                  & -23.8\%                               & 0.409                                 & 0.656                                  & -24.7\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{uob\_runid1}}       & 0.359                                 & 0.578                                  & -21.9\%                               & 0.389                                 & 0.670                                  & -28.0\%                               & 0.484                                 & 0.692                                  & -20.8\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{bl\_bcai\_multfld}} & 0.332                                 & 0.563                                  & -23.0\%                               & 0.399                                 & 0.685                                  & -28.6\%                               & 0.580                                 & 0.733                                  & -15.3\%                               \\ \hline
\multicolumn{1}{|l|}{\textbf{bcai\_classic}}     & 0.315                                 & 0.556                                  & -24.1\%                               & 0.376                                 & 0.642                                  & -26.6\%                               & 0.544                                 & 0.734                                  & -19.0\%                               \\ \hline
\end{tabular}
\end{table*}

==> tables/dl_hard_sparse.tex <==
\begin{table}[h]
\caption{Top systems on sparse \HARD judgements.}
\label{tab:dl_hard_sparse}
\begin{tabular}{l|r|r|}
\cline{2-3}
                                        & \multicolumn{1}{l|}{\textbf{NDCG@10}} & \multicolumn{1}{l|}{\textbf{RR}} \\ \hline
\multicolumn{1}{|l|}{uob\_runid3}       & 0.321                        & 0.500                   \\ \hline
\multicolumn{1}{|l|}{bcai\_bertb\_docv} & 0.409                        & 0.494                   \\ \hline
\multicolumn{1}{|l|}{bigIR-DT-T5-F}     & 0.286                        & 0.482                   \\ \hline
\multicolumn{1}{|l|}{bigIR-DTH-T5-F}    & 0.330                        & 0.460                   \\ \hline
\multicolumn{1}{|l|}{mpii\_run2}        & 0.328                        & 0.459                   \\ \hline
\multicolumn{1}{|l|}{mpii\_run1}        & 0.284                        & 0.435                   \\ \hline
\multicolumn{1}{|l|}{bigIR-DT-T5-R}     & 0.252                        & 0.428                   \\ \hline
\multicolumn{1}{|l|}{uogTrT20}          & 0.301                        & 0.425                   \\ \hline
\multicolumn{1}{|l|}{uob\_runid1}       & 0.337                        & 0.421                   \\ \hline
\multicolumn{1}{|l|}{uob\_runid2}       & 0.293                        & 0.414                   \\ \hline
\end{tabular}
\vspace{-4mm}
\end{table}


==> tables/entity_annotations.tex <==

\begin{table}[]
\caption{Question entity linking annotations.}%manual and automatic annotations.}
\label{tab:entity_annotations}
\begin{tabular}{l|r|r|}
\cline{2-3}
                                            & \textbf{2019} & \textbf{2020} \\ \hline
\multicolumn{1}{|l|}{Auto REL Links}             & 2             & 3             \\ \hline
\multicolumn{1}{|l|}{Auto GENRE Links}           & 101           & 111           \\ \hline
\multicolumn{1}{|l|}{Auto BLINK Links}           & 84            & 90            \\ \hline
\multicolumn{1}{|l|}{Auto ELQ Links}             & 89            & 102           \\ \hline
\multicolumn{1}{|l|}{Manual Links}            & 68            & 76            \\ \hline
\multicolumn{1}{|l|}{Answer in Link}        & 32            & 27            \\ \hline
\multicolumn{1}{|l|}{Core Entities in Wiki} & 42            & 39            \\ \hline
\end{tabular}
%\vspace{-4mm}
\end{table}

==> tables/judgments.tex <==
% \begin{table}[t]
%     \centering
%     \caption{\HARD\ Judgment Statistics}\label{tab:judgmentsstat}
%     \begin{tabular}{l|c|c|c|c}
%     \hline \hline
%     \textbf{Relevance} & \textbf{Doc} & \textbf{TREC Doc} & \textbf{TREC Passage} & \textbf{Passage}\\
%     \hline
%     0 & 33,781 *    & 5,164     & 2,403     & 292\\
%     1 & 2,697       & 2,498     & 707       & 379\\
%     2 & 1,834       & 454       & 570       & 149\\
%     3 & 1,408       & 309       & 305       & 189\\
    
%     \hline \hline
%     \end{tabular}
% \end{table}


\begin{table}[t]
    \centering
    \caption{\HARD\ Judgment statistics including DL labels and newly developed assessments.}\label{tab:judgmentsstat}
\begin{tabular}{|r|r|r|r|r|}
\hline
\multicolumn{1}{|l|}{\textbf{Rel. label}} & \multicolumn{1}{l|}{\textbf{DL Doc}} & \multicolumn{1}{l|}{\textbf{New Doc}} & \multicolumn{1}{l|}{\textbf{DL Psg}} & \multicolumn{1}{l|}{\textbf{New Psg}} \\ \hline
0                                        & 5,164                                & 145                                   & 2,403                                    & 292                                       \\ \hline
1                                        & 2,498                                & 180                                   & 707                                      & 379                                       \\ \hline
2                                        & 454                                  & 93                                    & 570                                      & 149                                       \\ \hline
3                                        & 309                                  & 146                                   & 305                                      & 189                                       \\ \hline
\end{tabular}
\end{table}

==> tables/query_intent_correlatation.tex <==
\begin{table}[h]
\caption{Query Intent Category Performance on DL 2019/20 Systems (Systems above medium).}
\begin{tabular}{l|r|r|r|r|r|r|}
\cline{2-7}
\label{query_intent:correlation}
                                            & \multicolumn{2}{c|}{\textbf{NDCG@10}}                                & \multicolumn{2}{c|}{\textbf{RR}}                                     & \multicolumn{2}{c|}{\textbf{Recall@100}}                             \\ \hline
\multicolumn{1}{|l|}{\textbf{Query Intent}} & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{r}} & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{r}} & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{r}} \\ \hline
\multicolumn{1}{|l|}{Attribute}             & 0.699                              & 0.10                            & 0.909                              & 0.08                            & 0.842                              & 0.22                            \\ \hline
\multicolumn{1}{|l|}{Description}           & 0.615                              & -0.02                           & 0.658                              & 0.01                            & 0.750                              & -0.04                           \\ \hline
\multicolumn{1}{|l|}{Entity}                & 0.567                              & -0.07                           & 0.646                              & -0.11                           & 0.616                              & -0.02                           \\ \hline
\multicolumn{1}{|l|}{Language}              & 0.778                              & 0.12                            & 0.677                              & 0.05                            & 0.862                              & 0.00                            \\ \hline
\multicolumn{1}{|l|}{List}                  & 0.568                              & -0.07                           & 0.466                              & -0.02                           & 0.726                              & -0.20                           \\ \hline
\multicolumn{1}{|l|}{Process}               & 0.758                              & 0.09                            & 0.867                              & -0.01                           & 0.727                              & 0.09                            \\ \hline
\multicolumn{1}{|l|}{Quantity}              & 0.594                              & -0.04                           & 0.675                              & 0.05                            & 0.791                              & 0.00                            \\ \hline
\multicolumn{1}{|l|}{Reason}                & 0.596                              & -0.03                           & 0.682                              & -0.05                           & 0.686                              & 0.01                            \\ \hline
\multicolumn{1}{|l|}{Verification}          & 0.691                              & 0.05                            & 0.863                              & -0.01                           & 0.726                              & 0.09                            \\ \hline
\multicolumn{1}{|l|}{Weather}               & 0.735                              & 0.05                            & 0.464                              & 0.05                            & 0.930                              & -0.06                           \\ \hline
\end{tabular}
\end{table}
